Categorising current-voltage curves in single-molecule junctions and their comparison to Single-Level Model

This thesis investigates the mechanically controlled break junctions, with a particular emphasis on elucidating the behaviour of molecular currents at room temperature. The core of this experimental investigation involves a detailed analysis of conductance, examining how it varies over time and with changes in the gap between electrodes. Additionally, this study thoroughly evaluates transmission properties, coupling effects, and current characteristics. A pivotal aspect of the research was the meticulous current measurement, followed by carefully selecting optimal data sets. This process set the stage for an in-depth analysis of resonant tunnelling phenomena observed through a single channel. Notably, these experiments were conducted under open atmospheric conditions at room temperature. A significant finding from this study is the recognition that our current model requires refinement. This adjustment is necessary to encapsulate a broader spectrum of molecular transport mechanisms more accurately. Furthermore, this work significantly advances our comprehension of quantum effects in single-molecule junctions, particularly concerning similar molecules to Corannulene extending to some organometallics. One of the essential disclosures is the identification of deviations in the transport model, primarily attributable to electron-electron interactions. This insight is crucial as it paves the way for developing a more comprehensive and precise model, enhancing our understanding of molecular-scale electronic transport.

==> bibliography_mcbj.tex <==

\bibliography{bibliography_mcbj.bib}
